Very ampleness of the canonical bundle of surfaces of type (1, 2, 2) on abelian threefolds

The present work deals with the canonical map of smooth, compact complex surfaces of general type in a polarization of type $(1,2,2)$ on an abelian threefold. A natural and classical question is whether the canonical system of such surfaces is very ample in the general case. In this work, we provide a positive answer to this question. First, we describe the structure of the canonical map of those smooth ample surfaces of type $(1,2,2)$ in an abelian threefold which are bidouble cover of principal polarizations. Then, we study the general behavior of the canonical map of general ample surfaces $\mathcal{S}$, yielding a $(1,2,2)$-polarization on an abelian threefold $A$ which is isogenous to a product. By combining these descriptions, we show that the canonical map yields a holomorphic embedding when $A$ and $\mathcal{S}$ are both sufficiently general. It follows, in particular, a proof of the existence of canonical irregular surfaces in $\mathbb{P}^5$ with numerical invariants $p_g = 6$, $q = 3$ and $K^2 = 24$.

==> Abelian1.tex <==
\section{Etale Abelian covers and torsion free sheaves}
\begin{prop1}
Let $V$ a complex vector space of dimenson $g \geq 1$ and $\Lambda$ a lattice in $V$. Let moreover $\Lambda'$ a sublattice of  $\Lambda$ and $G = \bigslant{\Lambda}{\Lambda'}$ a finite abelian group. Denote:
\begin{align*}
A = \bigslant{V}{\Lambda'} \\
B =  \bigslant{V}{\Lambda}
\end{align*}
and $p: A \longrightarrow B$ the natural projection.
Then we have:
\begin{equation*}
p_*{\mathcal{O}_A} \cong \bigoplus_{\chi \in G^*} \mathcal{L}_{\chi}
\end{equation*}
where $\mathcal{L}_{\chi}$ is the line bundle on $B$ associated (accordingly to Appel-Humbert theorem) to the semicharacter $\chi \circ q$ on $\Lambda$, where $q$ is the projection of $\Lambda$ onto $G$.
\end{prop1}
\begin{proof}
We call $\pi_B: V \longrightarrow B$ and $\pi_A: V \longrightarrow A$ the projections. The stalk of $p_*\mathcal{O}_A$, which has dimension $|G|$, is a $\C G$-module isomorphic to the regular representation.The trivial vector bundle $\pi_B^*(p_*\mathcal{O}_A)$ can be expressed then as:
\begin{equation*}
\pi_B^*(p_*\mathcal{O}_A) \cong \C[G]
\end{equation*}
where $\C[G]$ is the group algebra of $G$ over $\C$. The regular action of $G$ on $\C[G]$ (the action by left multiplication) decomposes as the sum:
\begin{equation*}
\C[G] \cong \bigoplus_{\chi \in G^*} W_{\chi}
\end{equation*}
where $W_{\chi}$ is the irreducible $\C[G]$-module of dimension $1$ associated to the character $\chi$. To the $\C[G]$-module $W_{\chi}$ is associated the line bundle $\bigslant{V \times W_{\chi}}{\sim_{\chi} }$ on $B$ where:
\begin{equation*}
(v, t) \sim_{\chi} (v + \lambda, q(\lambda).t) = (v + \lambda, (\chi \circ q)(\lambda)t)
\end{equation*}
But this is exactly the line bundle on $B$ associated (accordingly to Appel-Humbert theorem) to the semicharacter $\chi \circ q$ on $\Lambda$.
\end{proof}

Let us write $J = \bigslant{V}{\Lambda}$ a principally polarized abelian variety and $A = \bigslant{V}{\Lambda'}$ an abelian variety with $\Lambda'$ a sublattice of  $\Lambda$.
We have the projection $p: A \longrightarrow J$ and, accordingly with the previous proposition:
\begin{equation*}
p_*{\mathcal{O}_A} \cong \bigoplus_{\chi \in G^*} \mathcal{L}_{\chi}
\end{equation*}
We have then a copy of the group $G^*$ generated by the line bundles $\mathcal{L}_{\chi}$ immersed in $\widehat{J}$.

The polarization of $\widehat{J}$ is principal, and then the morphism $\phi_{\Theta}: J \longrightarrow \widehat{J}$ is an isomorphism. Then for every $\chi \in G^*$ there exists $g_{\chi} \in J$ such that:
\begin{equation*}
 \phi_{\Theta}(g_{\chi}) = \mathcal{O}_{J}(t_{g_\chi}^*\Theta) \otimes  \mathcal{O}_{J}(\Theta)^{-1} = \mathcal{L}_{\chi}
\end{equation*}
this means that, then:
\begin{equation} \label{projchar}
\chi \circ q = e^{2 \pi i E(g_{\chi}, \cdot)}
\end{equation}
where $q$ is the projection of $\Lambda$ into $G$. Howewer, is clear that:
\begin{equation*}
g_{\chi} + g_{\chi'} = g_{\chi \chi'}
\end{equation*}
And in particular we obtain that:
\begin{equation*}
G \cong \{g_{\chi} \ | \ \chi \in G^* \} \leq J
\end{equation*}
We obtain than $\Lambda_G$ a corresponding sublattice of $V$. Note, however, that for every $g \in \Lambda_G$ is defined:
\begin{align*}
\psi_{g}: \Lambda \longrightarrow \mathbb{S}^1 \\
\psi_{g}(\lambda) = e^{2 \pi i E(g, \lambda)} 
\end{align*}
For the equation \ref{projchar}, all those characters on $\Lambda$ have the sublattice $\Lambda'$ in the kernel. Let's us then define:
\begin{equation*}
\Lambda^G = \bigcap_{g \in \Lambda_G} Ker(\psi_g) = \{v \in V \ | \ E(v, \Lambda_G) \subseteq \Z  \}
\end{equation*}
and we have that $\Lambda'$ is a sublattice of $\Lambda^G$. But the converse is also true. Infact,
\begin{equation*}
G^* \cong \{\psi_g \ | g \in G\}
\end{equation*}
\begin{equation*}
\bigslant {\Lambda}{\Lambda^G} \cong G^*
\end{equation*}
All the characters of $G$ are trivial on the subgroup $H = \bigslant{\Lambda^G}{\Lambda'}$ of $G = \bigslant{\Lambda}{\Lambda'}$, and then we conclude that $H = \{1\}$. 
\subsection{The polarization}
Let us suppose as before $A$ a polarized abelian variety, with $\mathcal{L}$ an ample line bundle. Then we have an isogeny onto a principally polarized variety $p: A \longrightarrow J$, and an associated subgroup $G$ of $J$, with $\mathcal{L} = p^* \mathcal{O}_J(\Theta)$. 
The polarization is defined as:
\begin{align*}
\phi_{\mathcal{L}}(z) = p^*(\phi_{\theta}(z)) &= p^* (\mathcal{O}_J(t_z)(\Theta) \otimes \mathcal{O}(\Theta)^{-1}) \\
&= p^*\mathcal{L}(0, e^{2 \pi i E(z, \cdot)}) \\
&= \mathcal{L}(0, e^{2 \pi iE(z,\cdot)})
\end{align*}
Its kernel is:
\begin{align*}
Ker(\phi_{\mathcal{L}}) = \{\bar{v} \in \bigslant{V}{\Lambda^G} \ | \ e^{2 \pi i E(v, \lambda)} = 0 \ \ \forall \lambda \in \Lambda^G \}
\end{align*}
We have then that:
\begin{equation*}
Ker(\phi_{\mathcal{L}}) = \bigslant{\Lambda_G}{\Lambda^G}
\end{equation*}
To study the polarization and defining a suitable basis for the space of sections, I suppose:
\begin{equation*}
G \cong \Z_{s_1} \oplus \cdots \oplus \Z_{s_r}
\end{equation*}
with $s_i$ dividing the next.

\noindent The alternating bilinear form $E$ takes than on $\Lambda_G$ values in $\frac{1}{s_r^2} \Z$.
There must then exist $\eta_1 \cdots \eta_g, \delta_1 \cdots \delta_g$ generators of $\Lambda_G$ such that:
\begin{equation*}
E(\eta_i, \delta_i) =\frac{a_i}{s_r^2}
\end{equation*}
with $a_i$ integers dividing the next. 


\begin{lem1}
With $u_i$ orders of $\eta_i$ in $\Lambda_G$ modulo $\Lambda$ and $v_i$ orders of $\delta_i$ in $\Lambda_G$ modulo $\Lambda$, we have that:
\begin{align*}
a_i = \frac{s_r^2}{u_iv_i}
\end{align*}
\end{lem1}
\begin{proof}
In particular, since $s_r \eta_i \in \Lambda$ and $s_r \delta_i \in \Lambda$, and that:
\begin{equation*}
E(s_r \eta_i, \frac{s_r}{a_i} \delta_i ) = 1 
\end{equation*}
We obtain that $\frac{s_r}{a_i} \delta_i \in  \Lambda$ and $\frac{s_r}{a_i} \eta_i \in  \Lambda$. From this is clear that $\frac{s_r}{a_i}$ is a natural number, and $u_i$ divides $\frac{s_r}{a_i}$.
But we obtain even that:
\begin{equation*}
E(u_i\eta_i, v_i\delta_i) = 1  
\end{equation*}
and this means that:
\begin{equation*}
\frac{1}{u_i v_i} = \frac{a_i}{s_r^2}
\end{equation*}
\end{proof}
The order of $\eta_i$ in $\bigslant{\Lambda_G}{\Lambda^G}$ is then the same of the order of $\delta_i$, and this is exactly $u_iv_i$, since $\chi_{\eta_i}(u_iv_i \delta_i)=1$.
From this follows that the polarization of $A$ is exactly:
\begin{equation*}
(d_1 \cdots d_g) = (u_gv_g, \cdots u_1v_1)
\end{equation*}
\subsection{The basis of theta functions}

We take as a decomposition of $V$ for $\mathcal{L}$ the decomposition $V = V_1 \oplus V_2$, $V_1$ generated by $\delta_1 \cdots \delta_g$ and $V_2$ generated by $\eta_1 \cdots \eta_g$.
The decomposition distinguishes a semicharacter $\chi_0$ on $\Lambda$ whose extension on $V$ is:
\begin{equation*}
\chi_0(v) = e^{\pi i E(v_1, v_2)}
\end{equation*}
$H$ has no imaginary part  on $V_1$, and so $H$ is symmetric on $V_1$. Is then defined $B$ the $\C$-linear extension of $H|_{V_1 \times V_1}$ to $V$, because $V_1$ generates $V$ as $\C$-vector space. 
We have then:
\begin{equation*}
(H-B)(v,w) = \begin{cases}    0 \ \ \ \ \ \ \ \ \ \ \ \ \  \text{if} (v,w) \in V \times V_1 \\
				2iE(v,w) \ \   \text{if} (v,w) \in V_1 \times V
			\end{cases}
\end{equation*}
We have then that, with $v \in V_1$, $w \in V$:   
\begin{align*}
(H-B)(v,w) &=  \overline{H(w,v)} - B(w,v) \\
&=  \overline{H(w,v)} - B(w,v)  \\
&= \overline{H(w,v)} - H(w,v) \\
&= -2i E(w, v) = 2iE(v,w)
\end{align*}

Respect to the sum, $\chi_0$ behaves in the following way. Take $v$, $w$ in $V$. Then we have:
\begin{align*}
\chi_0(v+w) &= e^{\pi i E(v_1 + w_1, v_2 + w_2)} \\
&= \chi_0(v) \chi_0(w)e^{\pi i E(v_1, w_2) + \pi i E(w_1, v_2) } \\
&= \chi_0(v) \chi_0(w) e^{\pi i E(v,w) - 2 \pi i E(v_2, w_1)}
\end{align*}
Let us suppose that $\mathcal{O}_J(\Theta) = L(\chi_0, H)$, $\chi_0$ a semicharacter on $\Lambda$, namely, satysfing:
\begin{equation*}
\chi_0(\lambda + \mu) = \chi_0(\lambda)\chi_0(\mu)e^{\pi i E(\lambda, \mu) }
\end{equation*}
Then:
\begin{equation*}
\mathcal{L} = p^{*}(\mathcal{O}_J(\Theta) ) = p^{*}L(\chi_0, H) = L(\chi_0|_{\Lambda^G}, H)
\end{equation*}
Then I write the cocyles respect to this decomposition: with $v \in V$ we define
\begin{equation*}
\phi_{v}(z) = \chi_0(v) e^{\pi (H-B)(z, v) + \frac{\pi}{2}(H-B)(v, v)}
\end{equation*}
They satysfies, for every $u$, $v$ and $z$ in $V$ the following relation:
\begin{equation*}
\phi_{u+v}(z) = \phi_u(z+v)\phi_v(z)e^{\frac{\pi}{2}(H-B)(v,v) - \frac{\pi}{2}(H-B)(u,u)}
\end{equation*}
Indeed:
\begin{align*}
 & \phi_u(z+v)\phi_v(z) \\
 &= \chi_0(u)\chi_0(v)e^{\pi (H-B)(z+v, u) + \frac{\pi}{2}(H-B)(u, u)} e^{\pi (H-B)(z, v) + \frac{\pi}{2}(H-B)(v, v)}  \\
&=   \chi_0(u)\chi_0(v)e^{\pi (H-B)(z, v+u) + \pi (H-B)(v,u) + \frac{\pi}{2}(H-B)(u, u) +  \frac{\pi}{2}(H-B)(v, v)} \\
&=   \chi_0(u)\chi_0(v)e^{\pi (H-B)(z, v+u) + \frac{\pi}{2}  (H-B)(v+u,u) +  \frac{\pi}{2}(H-B)(v, v+u)} \\
&= e^{-\pi i E(u,v) + 2 \pi i E(u_2, v_1)}  \phi_{u+v}(z) e^{- \frac{\pi}{2}(H-B)(v+u,v) +  \frac{\pi}{2}(H-B)(v, v+u)} \\
&= e^{-\pi i E(u_1,v_2) +  -\pi i E(v_1,u_2) -  \pi i E(u_1,v_2) +  \pi i E(v_1, u_2)} \phi_{u+v}(z) \\
&=  e^{-2 \pi i E(u_1, v_2)}\phi_{u+v}(z)
\end{align*}
We define the theta functions: with $\eta \in {\Lambda_{G,2}}$:
\begin{equation*}
\theta^*[\eta](z) := \phi_{\eta}(z)^{-1}\theta(z+\eta)
\end{equation*}
\begin{lem1} \label{equalityactions}
For $g \in \Lambda$, we have:
\begin{equation*}
\theta^*[\eta](z+g) = e^{ - 2 \pi i E(g_1, \eta) } \phi_{g_2}(z) \theta^*[\eta](z) 
\end{equation*}
\end{lem1}
\begin{proof}
\begin{align*} 
\theta^*[\eta](z+g) &= \phi_{\eta}(z+g)^{-1}\theta(z+ \eta + g) \\
	&= \phi_{\eta}(z+g)^{-1} \phi_g(z+\eta) \theta(z+ \eta ) \\
	&= \phi_{\eta}(z+g)^{-1} \phi_g(z+\eta) \phi_{\eta}(z) \theta^*[\eta](z) \\
	&= \phi_{\eta}(z)^{-1} e^{-\pi(H-B)(g, \eta) } \phi_g(z+\eta) \phi_{\eta}(z) \theta^*[\eta](z) \\
	&=  e^{-\pi(H-B)(g, \eta) } \phi_g(z+\eta) \theta^*[\eta](z) \\
	&= e^{\pi(H-B)(\eta, g) -\pi(H-B)(g, \eta) } \phi_g(z) \theta^*[\eta](z) \\
	&=  e^{2 \pi i E(\eta_1, g_2) - 2 \pi i E(g_1, \eta_2) } \phi_{g_2}(z) \theta^*[\eta](z) \\
	&= e^{ - 2 \pi i E(g_1, \eta) } \phi_{g_2}(z) \theta^*[\eta](z)
\end{align*}
\end{proof}

This means in particular that $\theta^*[\eta]$ satisfies, for every $\mu \in \Lambda^{G}_2$:
\begin{equation*}
\theta^*[\eta](z+\mu) =  \phi_{\mu}(z) \theta^*[\eta](z)
\end{equation*}




%%BASIS OF THETA FUNCTIONS

\begin{prop1}
The sections $\theta^*[\eta]$, with $\eta \in \bigslant{\Lambda_{G,2}}{\Lambda^{G}_2 \cong G}$ give a basis for the sections of $H^0(A, \mathcal{L})$.
\end{prop1}
\begin{proof}
We observe first that, for every $\lambda \in \Lambda_1$ we have that:
\begin{equation*}
\phi_{\lambda}(z) \equiv 1
\end{equation*}
This means, in particular, that, for every $\eta \in \bigslant{\Lambda_{G,2}}{\Lambda^{G}_2}$ and $\lambda \in \Lambda_1$, we have:
\begin{align*}
\theta^*[\eta](z+\lambda) &=  \phi_{\eta}(z + \lambda)^{-1}\theta(z+\eta + \lambda) \\
					&= \phi_{\eta}(z) \theta(z+\eta) \phi_{\lambda}(z+\eta) \theta(z+\eta) \\
					&= \phi_{\eta}(z) \theta(z+\eta) \\
					& =\theta^*[\eta](z)
\end{align*}
Thus, $\theta^*[\eta]$ is periodic respect to $\Lambda_1$.
We can then write $\theta^*[\eta]$ in the following form:
\begin{equation*}
\theta^*[\eta](z) = \sum_{u \in \Lambda_{G,2}} \alpha_{u} e^{\pi (H-B) (z,u) }
\end{equation*}
If we take $\lambda \in \Lambda_2$, we obtain:
\begin{align*}
\phi_{\lambda}(z)\theta^*[\eta](z) = \theta^*[\eta](z + \lambda) &=  \sum_{u \in \Lambda_{G,2}} \alpha_{u} e^{\pi (H-B) (z+\lambda,u) } \\
&=	\sum_{u \in \Lambda_{G,2}} \alpha_{u} e^{\pi (H-B) (z ,u)}e^{\pi (H-B) (\lambda ,u) } 
\end{align*}
Thus:
\begin{align*}
\theta^*[\eta](z) &= \phi_{\lambda}(z)^{-1} \sum_{u \in \Lambda_{G,2}} \alpha_{u} e^{\pi (H-B) (z ,u)}e^{\pi (H-B) (\lambda ,u) } \\
&= e^{-\pi (H-B)(z,\lambda) - \frac{\pi}{2}(H-B)(\lambda, \lambda)} \sum_{u \in \Lambda_{G,2}} \alpha_{u} e^{\pi (H-B) (z ,u)}e^{\pi (H-B) (\lambda ,u) } \\
&= \sum_{u \in \Lambda_{G,2}} (\alpha_{u}  e^{- \frac{\pi}{2}(H-B)(\lambda, \lambda)})  e^{\pi (H-B) (z ,u - \lambda)}e^{\pi (H-B) (\lambda ,u) } \\
&= \sum_{u \in \Lambda_{G,2}} (\alpha_{u+\lambda}  e^{- \frac{\pi}{2}(H-B)(\lambda, \lambda)})  e^{\pi (H-B) (z ,u )}e^{\pi (H-B) (\lambda ,u+\lambda) } \\
&= \sum_{u \in \Lambda_{G,2}} (\alpha_{u+\lambda}  e^{\frac{\pi}{2}(H-B)(\lambda, \lambda)})  e^{\pi (H-B) (z ,u )}
\end{align*}
This means that the coefficient must only satisfy for every $u \in \Lambda_{G,2}$ and every $\lambda \in \Lambda_{2}$: 
\begin{equation*}
\alpha_{u+\lambda} = \alpha_{u} e^{- \frac{\pi}{2}(H-B)(\lambda, \lambda)}
\end{equation*}

\end{proof}
To conclude, let's study the action of 
\begin{equation*}
K(\mathcal{L}) = \bigslant{\Lambda_G}{\Lambda^G} = \bigslant{\Lambda_{G,1}}{\Lambda^G_1} \oplus \bigslant{\Lambda_{G,2}}{\Lambda^G_2}  \cong G \oplus G 
\end{equation*}
We have then:


\noindent For the second copy of $G$, lets take $g$ in $\Lambda_{G,2}$.
\begin{align*}
\theta^*[\eta](z+g) &= \phi_{\eta}(z+g)^{-1}\theta(z + \eta + g) \\
&= \phi_{\eta}(z+g)^{-1} \phi_{\eta + g}(z) \theta^{*}[\eta + g](z) \\
&= e^{\frac{\pi}{2}(H-B)(\eta,g) - \frac{\pi}{2}(H-B)(g,\eta) + \frac{\pi}{2}(H-B)(g,g)  }  e^{\pi(H-B)(z,g)} \theta^*[\eta+g](z) 
\end{align*}
For every $v$,$w$ in $V_2$, we have that:
\begin{equation*}
(H-B)(v,w) - (H-B)(w,v) = 0
\end{equation*}
Indeed, if $v = iv'$ and $w = iw'$, we have that:
\begin{align*}
(H-B)(v,w) - (H-B)(w,v) &= (H-B)(v,w) - (H-B)(w,v) \\
 &= (H-B)(iv',iw') - (H-B)(iw',iv') \\
 &=H(v',w')+ B(v',w') - H(w',v') - B(w',v') \\
 &=  H(v',w') - H(w',v') = H(v',w') - H(w',v') = 0
\end{align*}
So we conclude that, for every $g$ in $\Lambda_{G,2}$.
\begin{align*}
\theta^*[\eta](z+g) &= e^{ \frac{\pi}{2}(H-B)(g,g)  }  e^{\pi(H-B)(z,g)} \theta^*[\eta+g](z) 
\end{align*}


\subsection{Base points}
In this section let $A$ an abelian variety of dimension $g$ with $\mathcal{L}$ a symmetric ample line bundle of type $(d_1 \cdots d_g)$. Let $K(\mathcal{L})$ the kernel of the polarization:
\begin{equation*}
\phi_{\mathcal{L}} : A \longrightarrow \widehat{A}
\end{equation*}
The first observaton is the following: in $\zeta \in A$ is a base point for the linear system, then $-\zeta$ is again a base point (v. p. 91 Birkenhake, 6,4). However, the group $K(\mathcal{L})_2$ acts on the set of base points (see ex.2 p. 69 Birkenhake). Even the group $K(\mathcal{L})_1$ acts on this set, and th action of $K(\mathcal{L})$ is faithful on this set by translation.

Note that if $d_1 \geq 2$ then the system has no base points (the associated map is in this case a morphism), so suppose $d_1 = 1$. We have:
\begin{equation*}
\mathcal{L}^{n} = g! d_2 \cdot \cdots d_g
\end{equation*}
so, if the linear system has no fixed components, we have at most $n! d_2 \cdot \cdots d_g$ points.
On the other sides:
\begin{equation*}
K(\mathcal{L}) \cong \Z_{d_2}^2 \times \cdots \Z_{d_g}^2
\end{equation*}
So, in the case we have a linear system with base points and without fixed components, then there exist a natural $k \geq 1$ such that:
\begin{equation*}
kd_2^2 \cdots d_g^2 = |\mathcal{B}| 
\end{equation*}
and:
\begin{equation*}
g! d_2 \cdots d_g \geq |\mathcal{B}| =  kd_2^2 \cdots d_g^2 
\end{equation*}
so we conclude that with such a $k$ we have:
\begin{equation*}
g! \geq k d_2 \cdots d_g 
\end{equation*}
\subsection{Etale Abelian covers and curves}


Every curve will be considered to be nonsingular and projective over the field $\C$. We introduce the notion of abelian cover of curves by referring to the more general definition of abelian cover of algebraic variety as introduced in the article \cite{Pardini}.
\begin{def1}
Let $C$ a curve. \textbf{A cover of $C$ with group $G$} is a finite map $\pi: C' \longrightarrow C$ together with a faithful action of $G$ on $X$ such that $\pi$ exhibits $C$ as the quotient of $C'$ via $G$.
\end{def1}

\noindent Let us consider a curve $C$ of genus $g \geq 1$. We will denote always:
\begin{align*}
V &:= H^0(C, \omega_C)^{\vee} \\
\Lambda &:= H_1(C, \Z) 
\end{align*}
The abelian group $\Lambda$ will be considered as included in $V$ as a lattice via the integral operator. Moreover, we denote the Jacobian variety of $C$ as:
\begin{align*}
J(C) = \bigslant{V}{\Lambda}
\end{align*}
On $\Lambda$ is defined $E:  \Lambda \times \Lambda \longrightarrow \Z$ the bilinear alternating form given by the intersections of cycles, and with the same letter we refer us to its linear extension on $V$. $E$ is the alternating bilinear form of the principal polarization on $J(C)$ associated to the non-degenerate hermitian form $H: V \times V \longrightarrow \C$ defined from $E$ as following: 
\begin{equation*}
H(v,w) = iE(v,w) + E(iv,w)
 \end{equation*} 

Given an Etale abelian cover $\pi: C' \longrightarrow C$ of curves with group $G$, there exists a normal subgroup $H$ of $\pi_1(C)$ with quotient group $\bigslant{\pi_1(C)}{H}$ isomorphic to $G$ and, because $G$ is abelian, this group $H$ cooresponds to a sublattice $\Lambda'$ of $\Lambda$ with quotient isomorphic to $G$. The aim is then to construct a cartesian diagram of the type:
\begin{diagram} 
		C' 	&\rInto		& A	\\ 	
		 \dTo_{\pi} &							&\dTo_{p}			&				\\
		C			&\rInto			&J = J(C)
 \end{diagram}
 and determine the polarization of $A$. 
 
 \noindent Accordingly to the results contained in the article \cite{Pardini}, every such a cover is determined by a group of torsion bundles isomorphic to $G$ itself, and then it makes sense to consider first the $G$-covers of the Jacobian variety, $G$ an abelian group embedded in $J(C)$. 
 
\noindent Let $\Lambda_G$ be the corresponding lattice in $V$ with:
\begin{align*}
\Lambda \leq \Lambda_G \leq V \\
\bigslant{\Lambda_G}{\Lambda} \cong G
\end{align*}
We denote the isomorphism $\phi_{\Theta}: J(C) \longrightarrow Pic^0(J(C)) \cong Hom(\Lambda, \mathbb{S}^{1})$ associated to the polarization given by the Theta-divisor $\Theta$ of $C$:
\begin{align*}
\phi_{\Theta}: Pic^0(C) \cong &J(C) \longrightarrow Pic^0(J(C)) \cong Hom(\Lambda, \mathbb{S}^{1})\\
\phi_{\Theta}(x)&:=\mathcal{O}_{J(C)}(t_x^*\Theta) \otimes \mathcal{O}_{J(C)}(\Theta )^{-1}
\end{align*}
Given $x \in J(C)$, the line bundle $\phi_{\Theta}(x)$ on $J(C)$ is defined (respect to the Appel-Humbert theorem) by the semicharacter:
\begin{equation*}
e^{2 \pi i E(x, \cdot)}: \Lambda \longrightarrow \mathbb{S}^1 
\end{equation*}
We could consider the image in $Hom(\Lambda, \mathbb{S}^{1})$ of the group $G$ via $\phi_{\Theta}$: Given $g=[\mu] \in G$, the associated character $\chi_{g}: \Lambda \longrightarrow \mathbb{S}^1$ is defined by:
\begin{equation*}
 \chi_g(\lambda) = e^{2 \pi i E(\mu, \lambda)} 
\end{equation*}
\noindent We can then consider moreover:
\begin{equation*}
\Lambda^G = \bigcap_{g \in \Lambda_G} Ker(\chi_g) = \{v \in V \ | \ E(v, \Lambda_G) \subseteq \Z  \}
\end{equation*}
This is a sublattice of $\Lambda$ with quotient group $\bigslant{\Lambda}{\Lambda^G}$ canonically isomorphic to $G^*$, with isomorphism induced by:
\begin{align*}
\Phi: \Lambda \longrightarrow G^* \\
\Phi(\lambda)(g) = \chi_g(\lambda)
\end{align*}
which is surjective with kernel $\Lambda^G$.
We define then the complex torus:
\begin{equation*}
A^G := \bigslant{V}{\Lambda^G}
\end{equation*}
with the natural projection $p: A^G \longrightarrow J(C)$. 
In the next step we show that with the characters $\chi_g$ we can describe the decomposition of the sheaf $p_*\mathcal{O}_{A^G}$ in line bundles on $J(C)$. 


\begin{prop1} \label{mainproposition}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given $G$ finite subgroup di $J(C)$ there exists  up to isomorphism an unique Etale abelian abelian cover $\pi: C^{G} \longrightarrow C$ such that:
\begin{equation*}
\pi_*\mathcal{O}_G \cong \bigoplus_{g \in G} g 
\end{equation*}
This is moreover a pullback of a type:
\begin{diagram} 
		C^G 	&\rInto		& A^G	\\ 	
		 \dTo_{\pi} &							&\dTo_{p}			&				\\
		C			&\rInto			&J = J(C)
 \end{diagram}
where $A^G$ is an abelian variety, with polarization depending on the generators of $G$.
Conversely, every abelian Etale abelian cover $\pi: C' \longrightarrow C$ of group $G$ can be obtained in this way.
\end{prop1}
\begin{proof}
The second assertion follow from \cite{Pardini}, proposition 2.1 p. 199. We prove then the first.
Given the group $G$ in $J(C)$, and defined $A^G$ as before, we define $C^G$ as the pullback $C \times_{J} A^G$. From the previous proposition we have:
\begin{equation*}
p_*{\mathcal{O}_{A^G}} \cong \bigoplus_{\chi \in G^*} \mathcal{L}_{\chi}
\end{equation*}
where $\mathcal{L}_{\chi}$ is the line bundle on $J(C)$ associated to the semicharacter $\chi \circ q$ on $\Lambda$, where $q$ is the projection of $\Lambda$ onto $G$. But then $\chi \circ q$ belongs to the image of $\phi_{\Theta}$ in $Hom(\Lambda, \mathbb{S}^1)$. So there exists $g \in G$ such that:
\begin{equation*}
\mathcal{L}_{\chi} = \mathcal{O}_{J(C)}(t_g^*\Theta) \otimes \mathcal{O}_{J(C)}(\Theta )^{-1} = \phi_{\Theta}(g)
\end{equation*}
and we can write:
\begin{equation*}
p_*{\mathcal{O}_{A^G}} \cong \bigoplus_{g \in G} \phi_{\Theta}(g)
\end{equation*}
The restriction $|_C: Pic^0(J(C)) \longrightarrow Pic^0(C) \cong J(C)$ is an isomorphism and we have (see Birkenhake-Lange 11.3.5 p.329): 
\begin{equation*}
\phi_{\Theta}(g)|_C = g^{-1}
\end{equation*}
From this we can conclude the first point.
\end{proof}

==> casi_4.5.tex <==
%%%%%% CASI NELLA DIMOSTRAZIONE DELLA 4.5



Hence, we have the following cases:
\begin{itemize}
\item If $(\zc, \wc)$ belongs to $\Delta \cap X$ then, by \ref{intersectionslocusdef}, $P$ and $Q$ lie on $W_3$, with $\zc$ and $\wc$
of $2$ torsion on $E_3$. Thus, we have
\begin{equation*}
\wc = \zc \notin div (\theta^{\E_3}_{0}) \cup div (\theta^{\E_3}_{1}) \PUNKT
\end{equation*}
We can, in particular, consider the following holomorphic sections (see \ref{a12b12sections})
\begin{equation} \label{a12b12sectionsGENERALS}
\begin{split}
a_{12}(\xc, \yc, \tau) &:= \begin{vmatrix} \theta^{(12)}_{00}(\xc,\tau) &  \theta^{(12)}_{00}(\yc,\tau) \\  \theta^{(12)}_{11}(\xc,\tau) &  \theta^{(12)}_{11}(\yc,\tau) \end{vmatrix} \in H^0(S_{\mathcal{U},12} \times_{\mathcal{U}} S_{\mathcal{U},12}, \mathcal{M}_{\mathcal{U},12} \times_{\mathcal{U}} \mathcal{M}_{\mathcal{U},12} ) \\
b_{12}(\xc,\yc,\tau) &:= \begin{vmatrix} \theta^{(12)}_{01}(\xc,\tau) &  \theta^{(12)}_{01}(\yc,\tau) \\  \theta^{(12)}_{10}(\xc,\tau) &  \theta^{(12)}_{10}(\yc,\tau) \end{vmatrix} \in H^0(S_{\mathcal{U},12} \times_{\mathcal{U}} S_{\mathcal{U},12}, \mathcal{M}_{\mathcal{U},12}^{-} \times_{\mathcal{U}} \mathcal{M}_{\mathcal{U},12}^{-} ) \PUNKT
\end{split}
\end{equation}
and there exists a closed subscheme $Z$ of $S_{\mathcal{U},12} \times_{\mathcal{U}} S_{\mathcal{U},12}$ such that %% COMMENTO : UP TO SHRINKING U???
\begin{equation} \label{piBproperty1}
\pi_B(\widehat{\mathcal{Q}}) \subseteq \Delta_{12} \cup \Delta_{12}^{-} \cup Z \cup Z^{-} \subseteq div(a_{12}) \cap div(b_{12}) \BEISTRICH
\end{equation}
where $\Delta_{12}$ is the diagonal in $S_{\mathcal{U},12} \times_{\mathcal{U}} S_{\mathcal{U}, 12}$, $\Delta_{12}^{-} := (id \times (-1))\cdot \Delta_{12}$, and with:
\begin{equation}\label{Zproperty1}
Z|_{\tau_0} = \{(x, \iota_1(x)) \ \ | \ \ x \in S_{12} \} \PUNKT
\end{equation}
However, $\pi_B(\widehat{\mathcal{Q}}|_{\tau_0})$ does not intersect by hypothesis $\Delta_{12}^{-}$. Indeed, if it were the case, we would have that $\{P,Q\} \subseteq W_1 \cap W_2 \cap W_3$, because by hypothesis $P$ and $Q$ lie on $W_3$ by \ref{firstOssBXE}, and if $\yc = -\xc$, then they belong to $W_1 \cap W_2$.

Thus, we have that
\begin{equation*}
\pi_B(\widehat{\mathcal{Q}}) \subseteq \Delta_{12} \cup Z \cup Z^{-} \subseteq div(a_{12}) \cap div(b_{12}) \PUNKT
\end{equation*}
However, (by \ref{Zproperty1}) $Z|_{\tau_0} \cap \Delta_{12}|_{\tau_{0}} = \{(x,x) \in S_{12} \times S_{12} \ \ | \ \ x_1 \in E_1[2]  \}$, and hence we conclude that $P = Q$. This case, however, has already excluded.  
\item If $(\zc, \wc)$ belongs to $(\Delta \cap X)'$, we can simply change the representative for $Q$ by selecting $(\xc',\zc') := (\xc+(1,1), \zc+1)$, and the same conclusion follows by considering the previous case.
\item If $(\zc, \wc)$ belongs to $\Delta \cap X'$, then we may assume that $\zc = \wc \in div (\theta^{\E_3}_0)$, and we would have again, (see the proof of \ref{generalbehavior1}) that $P=Q$.
\item If $(\zc, \wc)$ belongs to $\Delta' \cap X$, we can simply change the representative for $Q$ by selecting $(\xc',\zc') := (\xc+(1,1), \zc+1)$, and the same conclusion follows by considering the previous case.
\end{itemize}


==> productelliptic.tex <==
\begin{oss1} (Degeneration to product of elliptic curves) \label{OssEllipticcurves} %%%%%%%%%%%%%%%%%%%%%%%%%%%%REMARK 
\noindentTX In the case in which $\tau_{12} = 0$ we have that $T$ is the product of three $2$ polarized elliptic curves $T = E_1 \times E_2 \times E_3$, where $E_j := \bigslant{\C}{\left<2, \tau_{jj} \right>}$ for every $j = 1,2,3$. 
For every couple of indices $(i,j)$ it is defines, as in \ref{projanddefinitionsofS}, an isogeny of degree $2$
\begin{equation*}
p_{ij}: E_i \times E_j \longrightarrow S_{ij}:=\bigslant{E_i \times E_j}{\left<e_i+e_j\right>} \BEISTRICH
\end{equation*}
%Clearly also $A$ maps onto $S_{ij}$ and we have the diagram:
%\begin{diagram} 
%		E_1 \times E_2 \times E_3 & \rTo 	&  &  	\\ 	
%		 \uTo_{\rho}& 		 \rdTo(5,2)	^{\phi}					&	  		&	 &	\\
%		 \C \times \PR^1 \times \PR^1  &  &  \rTo^{\bar{\Phi}}  & &  &\PR^{d-1} \\
%\end{diagram}
and there exists a line bundle $\mathcal{M}_{ij}$ on $S_{ij}$ such that 
\begin{equation*}
p_{ij}^*\mathcal{M}_{ij} \cong \mathcal{O}_{E_i}(2O_{E_i}) \boxtimes \mathcal{O}_{E_j}(2O_{E_j}) \PUNKT
\end{equation*}
Hence, it holds in particular
\begin{equation*}
{p_{ij}}_*( \mathcal{O}_{E_i}(2O_{E_i}) \boxtimes \mathcal{O}_{E_j}(2O_{E_j})) ={p_{ij}}_*p_{ij}^*\mathcal{M}_{ij} \cong \mathcal{M}_{ij} \oplus t_{\frac{\tau_i}{2}}^*\mathcal{M}_{ij} \PUNKT
\end{equation*}
We further denote the space of global holomorphic sections of these line bundles as follows (see also \ref{invandantiinvparts1}):
\begin{equation}\label{theta12presentation}
\begin{split}
H^0(S_{ij}, \mathcal{M}_{ij}) &= \left<\theta^{(ij)}_{00}, \theta^{(ij)}_{11} \right> \\
H^0(S_{ij}, t_{\frac{\tau_i}{2}}^*\mathcal{M}_{ij}) &= \left<\theta^{(ij)}_{10}, \theta^{(ij)}_{01} \right> \PUNKT
\end{split}
\end{equation}
We observe that the theta fuctions $\theta^{(ij)}_{hk}$ in \ref{theta12presentation} are product of the two theta functions of the 
form $\theta^{(i)}_{h}\theta^{(j)}_{k}$ where
%according to definition \ref{remarktheta},
\begin{equation*}
H^0(E_j, \mathcal{O}_{E_j}(2O_{E_j})) = \left< \theta^{(j)}_{0}, \theta^{(j)}_{1} \right> \PUNKT
\end{equation*}
\end{oss1}


==> skew.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{def1}\label{ANTISIMMsections} %%
Given an abelian variety $A = \bigslant{\C^g}{\Lambda}$, we see that every derivation defines a skew symmetric multiplication of sections. More precisely, denoted by $\mathcal{L}$ and $\mathcal{M}$ two ample line bundles, there is a natural multiplication map on the space of holomorphic sections:
\begin{equation*}
\mu \colon H^0(A, \mathcal{L}) \otimes H^0(A, \mathcal{M}) \longrightarrow H^0(A, \mathcal{L} \otimes \mathcal{M})
\end{equation*}
However, every derivation $\DER{v}{}$ defined by a vector $v$ according with the identification $\C^2 \cong H^0(A, T_A)$ defines a skew symmetric multiplication% $\bigwedge$
\begin{equation*}
\SKMULT{v} \colon H^0(A, \mathcal{L}) \land H^0(A, \mathcal{M}) \longrightarrow H^0(A, \mathcal{L} \otimes \mathcal{M})
\end{equation*}
defined by:
\begin{align*}
\SKMULT{v}(s \wedge t) &= \begin{vmatrix}
                              s & t \\
                              \DER{v}{s} & \DER{v}{t}
                             \end{vmatrix} = s \cdot \DER{v}{t} - \DER{v}{s} \cdot t
\end{align*}
It is easily seen that this map is well defined and $\SKMULT{v}(s \wedge t)$ is a holomorphic section of $H^0(A, \mathcal{L} \otimes \mathcal{M})$. To show this, let us assume that $[\{\phi_{\lambda}\}_{\lambda}]$ and $[\{\psi_{\lambda}\}_{\lambda}]$ are the factor of automorphy respectively corresponding to the ample line bundles $\mathcal{L}$ and $\mathcal{M}$. Let us consider two global holomorphic sections $s$ and $t$ of $\mathcal{L}$ and $\mathcal{M}$. Then we have, for every $z$ in $\C^g$ and every element $\lambda$ of the lattice $\Lambda$, that:
\begin{align*}
        \begin{vmatrix}
        s(z + \lambda)  & t(z + \lambda) \\
        \DER{v}{s}(z + \lambda)& \DER{v}{t}(z + \lambda)
        \end{vmatrix} &= 
        \begin{vmatrix}
        \phi_{\lambda}(z)s(z) & \psi_{\lambda}(z)t(z) \\
        \DER{v}{\phi_{\lambda}}(z)s(z) + \phi_{\lambda}(z)\DER{v}{s}(z)& \DER{v}{\psi_{\lambda}}(z)t(z) + \psi_{\lambda}(z)\DER{v}{t}(z)
        \end{vmatrix} \\
        &=\begin{vmatrix}
        \phi_{\lambda}(z)s(z) & \psi_{\lambda}(z)t(z) \\
         \phi_{\lambda}(z)\DER{v}{s}(z)& \psi_{\lambda}(z)\DER{v}{t}(z)
        \end{vmatrix} \\
        &=\phi_{\lambda}(z)\psi_{\lambda}(z)\begin{vmatrix}
        s(z) & t(z) \\
        \DER{v}{s}(z)&\DER{v}{t}(z)
        \end{vmatrix}        
\end{align*}
This proves the claim, since $[\{\phi_{\lambda}\cdot \psi_{\lambda}\}_{\lambda}]$ is the factor of automorphy of the line bundle $\mathcal{L} \otimes \mathcal{M}$.
\end{def1}
\begin{ex1}
Let us consider a $(2)$-polarized elliptic curve $\E = \bigslant{\C}{\left<\tau \Z \oplus 2\Z \right>}$. The elliptic curve $\E$ can be viewed as the Riemann surface defined in an affine neighborhood $\EU{}$ by an equation $\Eeq{} = 0$, where:
\begin{equation}\label{LegendreNormalForm}
\Eeq{} := \y{}^2 - (\x{}^2 - 1)(\x{}^2 - \pa{}^2) \PUNKT
\end{equation}%}
where ($\x{}$,$\y{}$) are the coordinates of an affine plane, and $\pa{}$ is a parameter which only depends on the element on $\tau$ %$\tau_{\E_j}$ in the Siegel half-plane defining $\E_j$. 
\noindentTX The affine model in (\ref{LegendreNormalForm}) is called the Legendre normal form of $\E_{}$ (see \cite{Catanese2016}). 


This Riemann surface defined by the equation $\Eeq{} = 0$ has two points at infinity, which we denote by $\inftyplus$ and $\inftyminus$ around which the function $\x{}$ has a simple pole. Thus, we can consider $\vinf{} := \frac{1}{\x{}}$ to be a local parameter around these points. Then, around these two points $\E$ can be viewed as defined in a neighborhood $\EV{}$ by an equation $\Eeqinf{} = 0$ in an affine plane with coordinates $(\vinf{}, \winf{})$, with
\begin{equation}\label{LegendreNormalForm2}
\Eeqinf{} := \winf{}^2 - (1 - \vinf{}^2)(1- \pa{}^2\vinf{}^{2}) \PUNKT
\end{equation}%}
The change of coordinates between $\EU{}$ and $\EV{}$ can be expressed as the map $(\x{}, \y{}) \mapsto (\vinf{}, \winf{}) = (\x{}^{-1},  \y{}\x{}^{-2})$.

\noindentTX The function $\x{j}$ defines a double cover of $\PR^1$ of degree $2$, which is ramified over the points of the set $\{1, -1, \pa{i}, -\pa{i}\}$. Such a double cover $\E \longrightarrow \PR^1$ has been called by Inoue a Legendre function for $\E$ (see \cite[p. 60]{BCatFrapp} and \cite{INOUE})). In general, a Legendre function $\LF$ on an elliptic curve $\E = \bigslant{\C}{\tau \Z \oplus 2 \Z}$ is a meromorphic function on $E$ which satisfies, for every point $z$ on $\E$, the following properties:
\begin{itemize}
\item $\LF(-z) = \LF(z)$.
\item $\LF \left(z+1\right) = -\LF(z)$.
\item $\LF \left(z+\frac{\tau}{2}\right) = \frac{\pa{}}{\LF{(z)}}$, $\LF(\frac{1}{2}) = -1$, $\LF(0) = 1$, $\LF(\frac{\tau}{2}) = \pa{}$, $\LF \left(\frac{1+\tau}{2}\right) = -\pa{}$.
\item  $\LF'(z) = 0$ if and only if $z \in \{0, 1, \frac{\tau}{2}, 1 + \frac{\tau}{2}  \}$. 
\end{itemize}
If we apply these properties to our situation we have that, since a Legendre function on an elliptic curve is unique, (see \cite[Lemma 3.2]{INOUE}):
\begin{equation} \label{LegendreRelationsEQ}
\frac{\theta^{\E_j}_0(0)\theta^{\E_j}_1(z)}{\theta^{\E_j}_1(0)\theta^{\E_j}_0(z)} = \x{j} \PUNKT
\end{equation}
Indeed, $\x{j}$ behaves as a Legendre function, while the left member satisfies all properties which characterize Legendre functions.

\noindentTX Note that the algebraic function $\y{j}$ corresponds in the analitic setting to the derivative of the Legendre function (up to a constant), which vanishes precisely on the set of $2$-torsion points of $\E_j$, and we have:

\begin{equation} \label{etadefinition_Y}
\y{j} \sim \eta_k := \begin{vmatrix}\theta^{E_j}_0 & \theta^{E_j}_1 \\ 
\frac{\partial}{\partial z_j} \theta^{E_j}_0 & \frac{\partial}{\partial z_j} \theta^{E_j}_1 \end{vmatrix} \in H^0(E_j, \OC_{E_j}(4O_{E_j})) \PUNKT
\end{equation}
\end{ex1}

